Rank-one matrix estimation: analytic time evolution of gradient descent dynamics

We consider a rank-one symmetric matrix corrupted by additive noise. The rank-one matrix is formed by an $n$-component unknown vector on the sphere of radius $\sqrt{n}$, and we consider the problem of estimating this vector from the corrupted matrix in the high dimensional limit of $n$ large, by gradient descent for a quadratic cost function on the sphere. Explicit formulas for the whole time evolution of the overlap between the estimator and unknown vector, as well as the cost, are rigorously derived. In the long time limit we recover the well known spectral phase transition, as a function of the signal-to-noise ratio. The explicit formulas also allow to point out interesting transient features of the time evolution. Our analysis technique is based on recent progress in random matrix theory and uses local versions of the semi-circle law.

==> app-diff-equ-genfunction.tex <==
\section{Proof of Lemma \ref{diff-equ-gen}}\label{app:diff-equ-genfunction}

blablabla

==> integro-differential-equations-ancien.tex <==
\section{Integro-differential equations}\label{integro-differential-equations}

We study gradient descent in a regime where $t = \tau n/\eta$, $n\to +\infty$, with $\tau$ fixed. Abusing slightly notation we set $\theta_{\tau n/\eta} \to \theta_{\tau}$ so that
equation \eqref{eq:mainode} reads
\begin{align}\label{eq:mainode2}
    \frac{d\theta_\tau}{d\tau} = -  n \nabla_\theta \mathcal H(\theta_\tau) + \theta_\tau \langle \theta_\tau, \nabla_\theta \mathcal H(\theta_\tau) \rangle
\end{align}

The matrix $H = \frac{\xi}{\sqrt n}$ is drawn at random from the Wigner GOE ensemble. For any small $\delta >0$, with probability tending to one as $n\to +\infty$, all eigenvalues fall in an interval $[-2 + \delta, 2 + \delta]$ \emph{refWigner}. Therefore, any contour $\mathcal{C} = \{z\in \mathbb{C} \mid z= \rho e^{i\theta}, \theta\in [0, 2\pi]\}$ with $\rho >2$, encircles the whole spectrum with probability tending to one when $n\to +\infty$, and we can define three generating functions
\begin{align}\label{eq:genfunctions}
Q_\tau(z) = \frac{1}{n}\langle \theta_\tau, \mathcal{R}_H(z) \theta^* \rangle, 
\quad
P_\tau(z) = \frac{1}{n}\langle \theta_\tau, \mathcal{R}_H(z) \theta_\tau \rangle,
\quad
R(z) = \frac{1}{n}\langle \theta^*, \mathcal{R}_H(z) \theta^* \rangle
\end{align}
where 

We define generalized overlaps  for all integer $k\in \mathbb{N}$, $q_k(\tau) = \frac{\langle \theta_\tau, H^k \theta^*\rangle}{n}$, $p_k(\tau) = \frac{\langle \theta_\tau, H^k \theta_\tau\rangle}{n}$, $r_k = \frac{\langle \theta^*, H^k \theta^*\rangle}{n}$ and first derive a hierarchy of coupled ODE's for the first two quantities. This then implies two integro-differential equations for their generating functions.

The gradient of the cost function is given by $\nabla_\theta \mathcal H(\theta_\tau) = -\frac{Y \theta_\tau}{n^2}$ so that:
\begin{equation}
    \frac{d\theta_\tau}{d\tau}  = \frac{1}{n^2} Y \theta_\tau
    - \frac{1}{n^2} \langle \theta_\tau, Y \theta_\tau \rangle \theta_\tau
\end{equation}
Using $Y = \theta^* \theta^{*T} + \frac{n}{\sqrt{\lambda}} H$ we have 
\begin{align}
    \frac{d \theta_\tau}{d\tau} & = 
    \frac{\langle \theta_\tau, \theta^*\rangle}{n}  \theta^*
    + \frac{1}{\sqrt \lambda} H \theta_\tau
    - \left( \frac{\langle \theta_\tau, \theta^* \rangle^2}{n^2} + 
      \frac{1}{\sqrt \lambda} \frac{\langle \theta_\tau, H \theta_\tau\rangle}{n}
    \right) \theta_\tau
    \nonumber \\ &
    =
    q_0(\tau)\theta^* + \frac{1}{\sqrt \lambda} H \theta_\tau  - \left( q_0(\tau)^2 + 
      \frac{p_1(\tau)}{\sqrt \lambda}
    \right) \theta_\tau
    \label{eq:continuity}
\end{align}
Hence it is clear that we must essentially solve for the objects $q_0(\tau)$ (the overlap at time $\tau$) and $p_1(\tau)$. 
Now, taking the inner product of each side of \eqref{eq:continuity} with  the vectors $n^{-1}H^k\theta^*$ and $n^{-1}H^k\theta_\tau$ respectively we get the following hierarchy of coupled ODE's
\begin{align}
    \begin{cases}
         \frac{dq_k}{d\tau} = q_0 r_k + \frac{1}{\sqrt \lambda} q_{k+1} - \left(q_0^2 + \frac{1}{\sqrt \lambda} p_1 \right) q_k
         \\
         \frac12 \frac{dp_k}{d\tau} = q_0 q_k + \frac{1}{\sqrt \lambda} p_{k+1} - \left(q_0^2 + \frac{1}{\sqrt \lambda} p_1 \right) p_k
        \end{cases}
    \label{eq:odes}
\end{align}
Here $k\in \mathbb{N}$ and we have omitted the $\tau$ dependence of $q_k(\tau)$, $p_k(\tau)$. 

We do not directly analyze this system but first introduce the following three generating functions. For $z\in \mathbb{C}\setminus \mathbb{R}$ let 
$\mathcal{R}_H(z) = (H - z I)^{-1}$ be the resolvent matrix (here $I$ is the identity $n\times n$ matrix) and let 
\begin{align}\label{eq:genfunctions}
Q_\tau(z) = \frac{1}{n}\langle \theta_\tau, \mathcal{R}_H(z) \theta^* \rangle, 
\quad
P_\tau(z) = \frac{1}{n}\langle \theta_\tau, \mathcal{R}_H(z) \theta_\tau \rangle,
\quad
R(z) = \frac{1}{n}\langle \theta^*, \mathcal{R}_H(z) \theta^* \rangle
\end{align}
From the standard representation from functional calculus \emph{Helfer-Sjostrand or other ref ?} we have for any circular contour $\mathcal{C} =\{z\in \mathbb{C}\mid \vert z\vert =\rho_n\}$ of radius 
$\rho_n>\Vert H\Vert_{\rm op}$, $H^k = - \int_{\mathcal{C}} \frac{dz}{2\pi i} z^k \mathcal{R}_H(z)$. 
Taking the inner products with the appropriate finite-dimensional vectors we get for any finite $n$ and $\tau$,
\begin{align}\label{eq:recovermoments}
q_k(\tau) = -\oint_{\mathcal{C}} \frac{dz}{2\pi i} z^k Q_\tau(z), \quad p_k(\tau) = -\oint_{\mathcal{C}} \frac{dz}{2\pi i} z^k P_\tau(z), \quad r_k(\tau) = -\oint_{\mathcal{C}} \frac{dz}{2\pi i} z^k R_\tau(z).
\end{align}
{\color{blue} Since all eigenvalues of a Wigner matrix fall in the interval $[-2, 2]$ with probability tending to one as $n\to \infty$ \cite{} this representation is valid with high probability as long as $R_n > 2$ and we can forget about the $n$-dependence of the contour.} 

We have
\begin{proposition}\label{diff-equ-gen}
For any $z\in \mathbb{C}\setminus \mathbb{R}$ the generating functions \eqref{eq:genfunctions} satisfy the integro-differential equation
\begin{align}\label{eq:integrodiff}
\begin{cases}
    \frac{d}{d\tau}Q_\tau(z) = q(\tau) R(z) 
                               + \frac{1}{\sqrt \lambda} (z Q_\tau(z) + q(\tau))
                                - \left(q^2(\tau) + \frac{1}{\sqrt \lambda} p_1(\tau) \right) Q_\tau(z) 
    \\
    \frac12 \frac{d}{d\tau} P_\tau(z) = q(\tau) Q_\tau(z) 
                                        + \frac{1}{\sqrt \lambda} (z P_\tau(z) + 1)
                                         - \left(q^2(\tau) + \frac{1}{\sqrt \lambda} p_1(\tau) \right) P_\tau(z)
\end{cases}
\end{align}
where $q(\tau) = -\oint_{\mathcal{C}} \frac{dz}{2\pi i} Q_\tau(z)$ and $p_1(\tau) = -\oint_{\mathcal{C}} \frac{dz}{2\pi i} z P_\tau(z)$. 
%Using \eqref{eq:recovermoments} we immedialtely get back \eqref{eq:odes} for $q_k(\tau), p_k(\tau), r_k(\tau)$. In particular we obtain 
%the overlap $q_0(\tau)$.
\end{proposition}
%\begin{proof}
%The derivation of \eqref{eq:integrodiff} is a direct application of \eqref{eq:continuity}.
%Details are found in appendix \ref{app:diff-equ-genfunction}.
%\end{proof}


==> main-aknowledgment.tex <==
\section*{Acknowledgment} 
The work of A. B has been supported by Swiss National Science Foundation grant no 200020 182517.


==> random_feature.tex <==
\section{Random Feature Model}
\subsection{Model description}
We now explore a similar approach in the case of a random feature model. 
The aim is not to be exhaustive, but to show the previous method can be adapted to somewhat similar learning problems. In particular, we propose to use practically the same model as described in \cite{mei2019generalization}; for which the literate already provides insightful formula for the test-error and train-error. Here again, we revisit the same problem through the gradient descent algorithm and show that it can also be tracked to some extent.

We define a data dimension $d\in\mathbb N^*$, pick-up a fixed $\beta \in \mathcal S_d(1)$, choose $N \in \mathbb N^*$ iid vectors $\theta_i \sim U(\mathcal S_d(\sqrt d))$, and a random vector $a \sim U(\mathcal S_N(\sqrt N))$. Assuming a standard activation function $\sigma$, we then sample $n \in \mathbb N^*$ data-points according to the following model:
\begin{eqnarray}
    x & \sim & \mathcal U(\mathcal S_d(\sqrt d))\\
    \epsilon & \sim & \mathcal N(0,1)\\
    y & = & \langle x, \beta \rangle + \epsilon\\
    \hat y & = & \sum_{i=1}^N a_i \sigma\left( \frac{\langle x, \theta_i \rangle}{\sqrt d} \right)
\end{eqnarray}
We assume that $Y = [y_1, \ldots, y_n]^T$ and $X = [x_1, \ldots, x_n]^T$ are the collected samples so that $Y = X \beta + \xi$, and further define $Z = (z_{i,j}) \in \mathbb C^{n \times N}$ such that $z_{i,j} = \sigma\left( \frac{\langle x_i, \theta_j \rangle}{\sqrt d} \right)$ and $\hat Y = Za$. We want to minimize the risk $\mathcal R(a)$ with a $\lambda$-penalization defined by:
$\mathcal R(a) = \frac{1}{2n} \norm{ Y - \hat Y }^2 + \lambda \frac{N}{2d} \norm{a}^2$.

The least-square estimator is given by $a_{\text{lse}} = (Z^T Z + \frac{N}{d}\lambda I)^{-1} Z^T Y$ but we are essentially interested in re-visiting the gradient descent algorithm. We consider again the quadratic decomposition with the constant $C_y=\frac{\norm{Y}^2}{2n}$:
\begin{equation}
    \mathcal R(a) = C_Y - \frac{1}{n} \langle X \beta, Z a\rangle 
    + \frac{1}{2n} \langle a, \left(Z^T Z + \textstyle \frac{nN}{d} \lambda \right) a \rangle
\end{equation}
We take into account pre-chosen fixed ratios $\psi_1,\psi_2$ such that $N=\psi_1 d$ and $n = \psi_2 d$.

\subsection{Gradient descent analysis}
We consider again a continuous version of the gradient descent where $a_0$ and $(a_t)_{t>0}$ is a solution of the differential equation: $\partial_t a_t = -\eta \nabla_a \mathcal R(a_t)$ with $\eta$ is a positive constant. Therefore $\partial_t a_t = \eta \frac{d}{n} \left( \frac{1}{d} Z^T Y -  \left(\frac{Z^T Z}{d} + \psi_1 \psi_2 \lambda I \right) a \right)$. As before, we define a kernel $H = \frac{Z^TZ}{d}$ the following functions for $k \in \mathbb N$: $q_k(t) = \langle \frac{Z^T Y}{d}, H^k a_t \rangle$ and $p_k(t) = \langle a_t, H^k a_t \rangle$ and the constant $r_k = \langle \frac{Z^T Y}{d}, H^k \frac{Z^T Y}{d} \rangle$. The risk at time $t$ can be written as a combination: $\mathcal R(a_t) = C_Y - \frac{1}{\psi_2} \left(q_0(t) - \frac12 (p_1(t) + \lambda \psi_1 \psi_2 p_0(t)) \right)$ and it is thus desirable to find a system of ODE for $(q_0,p_1,p_0)$.

As before, choosing a constant $\eta = \psi_2$ we can develop a hierarchy of equations for all $k \in \mathbb N$:
\begin{equation}
    \left\{
    \begin{matrix}
        \partial_t q_k(t) & = & r_k - q_{k+1}(t) - \lambda \psi_1 \psi_2 q_k(t)\\
        \frac12 \partial_t p_k(t) & = & q_k(t) - p_{k+1}(t) - \lambda \psi_1 \psi_2  p_k(t)
    \end{matrix}
    \right.
\end{equation}
Thus, for $z \in \mathbb C$ and provided that $|z|>\norm{H}_{\text{op}}$, we can also naturally define for $t \in \mathbb R_+$:
\begin{equation}
    Q_t(z) = \sum_{k\geq 0} q_k(t) \frac{-1}{z^{k+1}} = 
    \langle \textstyle \frac{Z^T Y}{d}, (H - zI)^{-1} a_t \rangle  
    \label{eq:Q_rf}
\end{equation}
and similarly with $P_t(z)$ for $(p_k(t))_{k\geq 0}$ and $R(z)$ for $(r_k)_{k\geq 0}$. We thus have quite similar ODE:
\begin{equation}
    \left\{
    \begin{matrix}
        \partial_t Q_t(z) = R(z) - (z + \lambda \psi_1 \psi_2) Q_t(z) - q_0(t)\\
        \frac12 \partial_t P_t(z) = Q_t(z) - (z + \lambda \psi_1 \psi_2) P_t(z) - p_0(t)
    \end{matrix}
    \right.
    \label{eq:rf_ode}
\end{equation}

\subsection{Limiting-average case analysis}
We show that we can consider the asymptotic case as in the previous spiked wigner model. We thus consider the ODE Eq. \ref{eq:rf_ode} for $(\bar Q_t(z), \bar P_t(z))$ with initial conditions $(\bar Q_0(z), \bar P_0(z))$ and $\bar R(z)$ given the limit when $d \to \infty$ and averaged on $a_0$ and $\beta$.

Firstly, we notice that by independence of $a_0$ with $Z,H,Y,\beta$ in Eq. \ref{eq:Q_rf}, we obviously have for all $d \in \mathbb N$ that $\mean_{a_0}[Q_0(z)] = 0$ and hence we take $\bar Q_0(z) = 0$. Secondly, for $P_0(z)$ we have:
\begin{equation}
    \mean_{a_0}[P_0(z)] 
    = \trace{(H-zI)^{-1} \mean_{a_0}[a_0 a_0^T]} 
    = \trace{(H-zI)^{-1}}
\end{equation}
Eventually, for $R(z)$ we let $Q = \frac{XX^T}{d}$ and average on $\beta \sim \mathcal U ( \mathcal S_d(1) )$:
\begin{equation}
    \mean_{\beta}[R(z)] 
    = \trace{ (H-zI)^{-1} \textstyle \frac{Z^T}{d} X \mean_{\beta}[\beta \beta^T] X^T \textstyle \frac{Z}{d}} 
    = \trace{(H-zI)^{-1} \textstyle \frac{Z^T}{d} Q \textstyle \frac{Z}{d} }
\end{equation}

The value of $\bar P_0(z)$ and $\bar R(z)$ are given as a solution of order 4 polynomial as described in \cite{mei2019generalization}.
This allows us to construct an empirical spectral density $\mu_{\bar R}$ and $\mu_{\bar P_0}$ out of the inversion formula of the Stieltjes transform:
\begin{equation}
    \mu_{\bar R}(u) = \frac{-1}{\pi} \lim_{\epsilon \to 0^+} \Im(\bar R(u + i \epsilon))
\end{equation} 


\subsection{Dynamic risk analysis}

We solve Eq. \ref{eq:rf_ode} for $\bar Q_t, \bar P_t, \bar R$ with a similar approach as before: we use a Laplace transform over $t$ and get:
\begin{equation}
    p \mathcal L \bar Q_p(z) - \bar Q_0(z) = \frac{1}{p} \bar R(z) - (z+\lambda \psi_1 \psi_2) \mathcal L \bar Q_p(z) - \mathcal L \bar q_0(p)
\end{equation}
But using the previous fact that $\bar Q_0(z)= 0$, and choosing a contour $\Gamma$ such that for all $z \in \Gamma$, $|z| < \lambda \psi_1 \psi_2 + p$ and inverting laplace transform and contour integrals we have with $\lambda^* = \lambda \psi_1 \psi_2$:
\begin{equation}
    \mathcal Lq_0(p) = \frac{-1}{2i\pi} \oint_\Gamma 
    \frac{\bar R(z) \dd z}{p(p+z+\lambda^*)} 
\end{equation}
So, noticing that $\mathcal L\left( \frac{1 - e^{-t(z+\lambda^*)}}{z + \lambda^*} \right) = \frac{1}{p(p+z+\lambda^*)}$, and through an inverse Laplace transform, we get:
\begin{equation}
    q_0(t) = \int_{\mathbb R} \frac{1 - e^{-t (u+\lambda^*)}}{u + \lambda^*} \mu_{\bar R}(u) \dd u
\end{equation}

Similarly, we have:
\begin{equation}
    \mathcal L \bar P_p(z) = 
    \frac{1}{\frac12 p + z + \lambda^*} \left[
        \frac12 \bar P_0(z) +
        \mathcal L \bar Q_p(z) - \mathcal L \bar p_0(p)
    \right]
\end{equation}
and calculations lead to:
\begin{eqnarray}
    p_0(t) & = & \int_{\mathbb R} e^{-2t(u+\lambda^*)} \mu_{\bar P_0}(u) \dd u
    + \int_{\mathbb R} \left(\frac{1 - e^{-t (u+\lambda^*)}}{u + \lambda^*}\right)^2 \mu_{\bar R}(u) \dd u \\
    p_1(t) & = &
    \int_{\mathbb R} u e^{-2t(u+\lambda^*)} \mu_{\bar P_0}(u) \dd u
    + \int_{\mathbb R} u \cdot \left(\frac{1 - e^{-t (u+\lambda^*)}}{u + \lambda^*}\right)^2 \mu_{\bar R}(u) \dd u
\end{eqnarray}
and we can finally retrieve the risk at all time $t$:
\begin{equation}
    \mathcal R(a_t) = C_Y + 
    \frac{1}{\psi_2} \int_{\mathbb R} (u + \lambda^*) e^{-2t(u+\lambda^*)} \mu_{\bar P_0}(u) \dd u -
    \frac{1}{\psi_2} \int_{\mathbb R} \frac{1 - e^{-2 t (u+\lambda^*)}}{u + \lambda^*} \mu_{\bar R}(u) \dd u
\end{equation}

==> settings_custom.tex <==
% new commands
\newcommand*\NewPage{\null\thispagestyle{empty}\newpage}
\def \L{{\cal L}}
\def \({\left(}
\def \){\right)}
\def \[{\left[}
\def \]{\right]}
\def \nn{\nonumber \\}
\newcommand{\tbf}[1]{{\textbf{#1}}}
\newcommand{\bsy}[1]{{\boldsymbol{#1}}}
\newcommand{\txt}[1]{\text{#1}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\newcommand{\cv}[1]{\underline{#1}}
\newcommand{\bQ}{{\bm {Q}}}
\newcommand{\bq}{{\bm {q}}}
\newcommand{\br}{{\bm {r}}}
\newcommand{\bF}{{\bm {F}}}
\newcommand{\bY}{{\bm {Y}}}
\newcommand{\bff}{{\bm {f}}}
\newcommand{\bG}{{\bm {G}}}
\newcommand{\bU}{{\bm {U}}}
\newcommand{\bV}{{\bm {V}}}
\newcommand{\bW}{{\bm {W}}}
\newcommand{\bZ}{{\bm {Z}}}
\newcommand{\bh}{{\bm {h}}}
\newcommand{\bw}{{\bm {w}}}
\newcommand{\bv}{{\bm {v}}}
\newcommand{\bg}{{\bm {g}}}
\newcommand{\bA}{{\bm {A}}}
\newcommand{\bB}{{\bm {B}}}
\newcommand{\bC}{{\bm {C}}}
\newcommand{\bhx}{\hat {\bm {x}}}
\newcommand{\bX}{{\bm {X}}}
\newcommand{\bx}{{\bm {x}}}
\newcommand{\bo}{{\bm {o}}}
\newcommand{\blambda}{{\boldsymbol{\Lambda}}}
\newcommand{\btau}{{\boldsymbol{\tau}}}
\newcommand{\by}{{\bm {y}}}
\newcommand{\bz}{{\bm {z}}}
\newcommand{\bl}{{\bm {l}}}
\newcommand{\bs}{{\bm {s}}}
\newcommand{\bu}{{\bm {u}}}
\newcommand{\bS}{{\bm {S}}}
\newcommand{\bc}{{\bm {c}}}
\newcommand{\bk}{{\bm {k}}}
\newcommand{\bR}{{\bm {R}}}
\newcommand{\beps}{{\boldsymbol {\epsilon}}}
\newcommand{\bxigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bxi}{{\boldsymbol{\xi}}}
\newcommand{\bzero}{{\textbf{0}}}
\newcommand{\ba}{{\bm {a}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\lab}[1]{\label{#1}}
\newcommand{\bxii}{{\boldsymbol{\xi}}}
\newcommand{\bre}{{\bm {e}}}
\newcommand{\bytilde}{{\tilde{\bm {y}}}}
\newcommand{\bxhat}{{\tilde{\bm {x}}}}
\newcommand{\mc}{\mathcal}
\newcommand{\eps}{\varepsilon}
\newcommand{\calF}{\mathcal F}
\newcommand{\s}{\sigma}
\renewcommand{\d}{\text{d}}
\newcommand{\e}{\text {e}}
\newcommand{\ds}{\Delta\sigma}
\newcommand{\hw}{h^{\rm W}}
\newcommand{\sw}{\sigma^{\rm W}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\de}{\partial}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\eq}{\text{ eq}}
\newcommand{\sign}{\text{ sign}}
\newcommand{\ua}{\uparrow}
\newcommand{\da}{\downarrow}
\newcommand\smallO{
  \mathchoice
    {{\scriptstyle\mathcal{O}}}% \displaystyle
    {{\scriptstyle\mathcal{O}}}% \textstyle
    {{\scriptscriptstyle\mathcal{O}}}% \scriptstyle
    {\scalebox{.7}{$\scriptscriptstyle\mathcal{O}$}}%\scriptscriptstyle
  }

\DeclareMathOperator{\atanh}{atanh}
\DeclareMathAlphabet{\varmathbb}{U}{bbold}{m}{n}
\newcommand{\id}{\mathds{1}}
%\newcommand{\noi}{\noindent}
\renewcommand{\d}{{\rm d}}
\renewcommand{\P}{{\rm P}}
\newcommand{\B}{{\rm B}}
\newcommand{\Tr}{{\rm Tr}}
\newcommand{\iif}{\Longleftrightarrow}

